Improving VTE Identification through Language Models from Radiology Reports: A Comparative Study of Mamba, Phi-3 Mini, and BERT

Venous thromboembolism (VTE) is a critical cardiovascular condition, encompassing deep vein thrombosis (DVT) and pulmonary embolism (PE). Accurate and timely identification of VTE is essential for effective medical care. This study builds upon our previous work, which addressed VTE detection using deep learning methods for DVT and a hybrid approach combining deep learning and rule-based classification for PE. Our earlier approaches, while effective, had two major limitations: they were complex and required expert involvement for feature engineering of the rule set. To overcome these challenges, we utilize the Mamba architecture-based classifier. This model achieves remarkable results, with a 97\% accuracy and F1 score on the DVT dataset and a 98\% accuracy and F1 score on the PE dataset. In contrast to the previous hybrid method on PE identification, the Mamba classifier eliminates the need for hand-engineered rules, significantly reducing model complexity while maintaining comparable performance. Additionally, we evaluated a lightweight Large Language Model (LLM), Phi-3 Mini, in detecting VTE. While this model delivers competitive results, outperforming the baseline BERT models, it proves to be computationally intensive due to its larger parameter set. Our evaluation shows that the Mamba-based model demonstrates superior performance and efficiency in VTE identification, offering an effective solution to the limitations of previous approaches.

==> background.tex <==
\section{Background} \label{background}

\subsection{VTE Disease}

    \begin{figure}[t] 
    % * after figure, to span cross two columns
        \centering        \includegraphics[width=0.40\textwidth]{figs/vte.jpg}
        \caption{Venous Thromboembolism (Blood Clots).}
        \label{fig:vte}
    \end{figure}


Venous thromboembolism (VTE) is a serious and prevalent cardiovascular condition that encompasses deep vein thrombosis (DVT) and pulmonary embolism (PE). DVT occurs when a blood clot forms in the deep veins, as shown in Figure \ref{fig:vte}, typically in the lower extremities, while PE results when a clot dislodges and travels to the lungs, obstructing pulmonary arteries. VTE is a major contributor to morbidity and mortality worldwide and is particularly concerning in post-surgical patients, where the risk of clot formation can increase substantially. Despite advancements in medical care, the timely and accurate identification of VTE remains a significant challenge due to its often subtle clinical presentation and the need for rapid intervention to prevent life-threatening complications.

The complexity of diagnosing VTE lies in its reliance on various forms of clinical data, including imaging, laboratory results, and patient histories. Radiology reports, in particular, are essential in confirming the presence of DVT or PE, but interpreting these unstructured text documents demands significant expertise and time. Traditionally, VTE diagnosis has depended heavily on radiologists and clinicians meticulously reviewing medical reports, leading to variability in detection and delays in diagnosis. This variability underscores the pressing need for automated systems that can assist in identifying VTE with speed and consistency.

Incorporating artificial intelligence (AI) models into the detection of VTE offers a transformative solution to these challenges. AI, specifically natural language processing (NLP) models, can be trained to analyze free-text radiology reports, extracting crucial information that indicates the presence of VTE. These models have the potential to standardize the diagnostic process by reducing human error, increasing the speed of analysis, and providing consistent outputs based on extensive training on clinical datasets. Moreover, AI models can handle large volumes of data in real-time, making them indispensable in high-demand clinical environments where rapid decision-making is critical. The adoption of AI for VTE detection is not merely about improving accuracy; it is about optimizing the entire diagnostic workflow, enabling healthcare providers to intervene earlier and more effectively, thereby improving patient outcomes.
